Deep Attentional Guided Image Filtering

Guided filter is a fundamental tool in computer vision and computer graphics which aims to transfer structure information from guidance image to target image. Most existing methods construct filter kernels from the guidance itself without considering the mutual dependency between the guidance and the target. However, since there typically exist significantly different edges in the two images, simply transferring all structural information of the guidance to the target would result in various artifacts. To cope with this problem, we propose an effective framework named deep attentional guided image filtering, the filtering process of which can fully integrate the complementary information contained in both images. Specifically, we propose an attentional kernel learning module to generate dual sets of filter kernels from the guidance and the target, respectively, and then adaptively combine them by modeling the pixel-wise dependency between the two images. Meanwhile, we propose a multi-scale guided image filtering module to progressively generate the filtering result with the constructed kernels in a coarse-to-fine manner. Correspondingly, a multi-scale fusion strategy is introduced to reuse the intermediate results in the coarse-to-fine process. Extensive experiments show that the proposed framework compares favorably with the state-of-the-art methods in a wide range of guided image filtering applications, such as guided super-resolution, cross-modality restoration, texture removal, and semantic segmentation.

==> Deep Attentional Guided Image Filtering/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Deep Attentional Guided Image Filtering/abl_map.tex <==
\begin{figure}[!tb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{guide_att.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[$\bm{A}_0$]{
    		\begin{minipage}[b]{0.24\linewidth}
  		 	\includegraphics[width=1\linewidth]{guide_map_0.jpg}
    		\end{minipage}
    		\hspace{-0.1in}
    	}\subfigure[$\bm{A}_1$]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{guide_map_1.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[$\bm{A}_2$]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{guide_map_2.jpg} 
		\end{minipage}
	}
	\subfigure[Target]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{depth_att.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[$\bm{1} - \bm{A}_0$]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{depth_map_0.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[$\bm{1}- \bm{A}_1$]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{depth_map_1.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[$\bm{1} - \bm{A}_2$]{
		\begin{minipage}[b]{0.24\linewidth}
			\includegraphics[width=1\linewidth]{depth_map_2.jpg} 
		\end{minipage}
	}
    \includegraphics[width=0.97\linewidth]{bar.jpg} 
	\end{center}
% 	\vspace{-0.2in}
	 \caption{\textbf{Ablation Study}. Visualization of the learned multi-scale attention maps for kernel combination. We resize the attention map to the same size for better Visualization. Please enlarge the PDF for more details.}
	\label{fig:abl_map}
\end{figure}

==> Deep Attentional Guided Image Filtering/abl_res.tex <==
\begin{figure*}[!htb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.16\linewidth}
			\includegraphics[width=1\linewidth]{rgb_res.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Model1]{
    		\begin{minipage}[b]{0.16\linewidth}
  		 	\includegraphics[width=1\linewidth]{M2.jpg}
    		\end{minipage}
    		\hspace{-0.09in}
    	}\subfigure[Model2]{
		\begin{minipage}[b]{0.16\linewidth}
			\includegraphics[width=1\linewidth]{M1.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Model3]{
		\begin{minipage}[b]{0.16\linewidth}
			\includegraphics[width=1\linewidth]{M3.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Model4]{
		\begin{minipage}[b]{0.16\linewidth}
			\includegraphics[width=1\linewidth]{M4.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Model5]{
		\begin{minipage}[b]{0.16\linewidth}
			\includegraphics[width=1\linewidth]{dagf_res.jpg} 
		\end{minipage}
	}
	\end{center}
% 		\vspace{-0.1in}
    \caption{\textbf{Ablation Study}. Visual comparison of an example without and with the proposed attentional kernel learning module (AKL) for depth image super-resolution. The first row shows the super-resolved depth images and the last row shows the error map ($\bm{I}^{\text{h}} - \bm{I}^{\text{out}}$). Please enlarge the PDF for more details.}
	\label{fig:abl_res}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig1.tex <==
\begin{figure*}[!tb]
	\begin{center}
		\subfigure[Guidance Image]{
		\begin{minipage}[b]{0.19\linewidth}
			\includegraphics[width=1\linewidth]{rgb_img.jpg} 
		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_1}
	}\subfigure[GF]{
    		\begin{minipage}[b]{0.19\linewidth}
  		 	\includegraphics[width=1\linewidth]{gf_img.jpg}
    		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_2}
    	}\subfigure[JBU]{
		\begin{minipage}[b]{0.19\linewidth}
			\includegraphics[width=1\linewidth]{jbu_img.jpg} 
		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_3}
	}\subfigure[MuGF]{
    		\begin{minipage}[b]{0.19\linewidth}
  		 	\includegraphics[width=1\linewidth]{muf_img.jpg}
    		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_2}
    	}\subfigure[CUNet]{
		\begin{minipage}[b]{0.19\linewidth}
			\includegraphics[width=1\linewidth]{cu_img.jpg} 
		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_3}
	}
	\subfigure[DJFR]{
		\begin{minipage}[b]{0.19\linewidth}
			\includegraphics[width=1\linewidth]{djfr_img.jpg} 
		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_3}
	}\subfigure[PAC]{
		\begin{minipage}[b]{0.19\linewidth}
			\includegraphics[width=1\linewidth]{pac_img.jpg} 
		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_3}
	}\subfigure[DKN]{
    		\begin{minipage}[b]{0.19\linewidth}
		 	\includegraphics[width=1\linewidth]{dkn_img.jpg}
    		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_4}
    	}\subfigure[Ours]{
    		\begin{minipage}[b]{0.19\linewidth}
  		 	\includegraphics[width=1\linewidth]{our_img.jpg}
    		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_2}
    	}\subfigure[Ground Truth]{
    		\begin{minipage}[b]{0.19\linewidth}
  		 	\includegraphics[width=1\linewidth]{gt_img.jpg}
    		\end{minipage}
		%\label{fig:grid_4figs_1cap_4subcap_2}
    	}
	\end{center}
% 	\vspace{-0.1in}
	\caption{Guided image filtering on a RGB/D image pair for 16 $\times$ guided super-resolution: (a) Guidance image, (b) GF~\cite{GF}, (c) JBU~\cite{JBU}, (d) MuGF~\cite{mugf}, (e) CUNet~\cite{CUNet}, (f) DJFR~\cite{DJFR}, (g) PAC~\cite{PanNet}, (h) DKN~\cite{DKN}, (i) Ours, (j) Ground truth.  The results of (b)-(c) suffer from edge blurring artifact and the results of (d)-(h) suffer from texture-copying artifacts. Our result produces much sharper edges. Please enlarge the PDF for more details.}
	\label{fig:fm}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig1_1.tex <==
\begin{figure*}[!tb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.15\linewidth}
			\includegraphics[width=1\linewidth]{1.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[JBU]{
    		\begin{minipage}[b]{0.1\linewidth}
  		 	\includegraphics[width=1\linewidth]{2.jpg}
    		\end{minipage}
    		\hspace{-0.089in}
    	}\subfigure[GF]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{3.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[DMSG]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{4.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[DJFR]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{5.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[PAC]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{6.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[DKN]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{7.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{8.jpg} 
		\end{minipage}
		\hspace{-0.089in}
	}\subfigure[GT]{
		\begin{minipage}[b]{0.1\linewidth}
			\includegraphics[width=1\linewidth]{9.jpg} 
		\end{minipage}
	}
	\end{center}
% 	\vspace{-0.1in}
	\caption{Qualitative comparison for recovered depth maps (8×). (a) Guidace image, (b): JBU~\cite{JBU}, (c): GF~\cite{GF}, (d): DMSG~\cite{DMSG}, (e): DJFR~ \cite{DJFR}, (f): PAC~\cite{PanNet}, (g): DKN~\cite{DKN}, (h): DAGF, and (i) Ground truth depth map. Top to bottom: Each two rows present recovered depth maps on the NYU v2~\cite{NYU}, Sintel~\cite{Sintel}, Lu~\cite{Lu} and Middlebury~\cite{middleblur_data_1} datasets respectively. Please enlarge the PDF for more details.}
	\label{fig:fig_all}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig_cd.tex <==
\begin{figure}[!tb]
	\begin{center}
		\subfigure[~]{
		\begin{minipage}[b]{0.5\linewidth}
			\includegraphics[width=0.85\linewidth]{clean_rmse.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[~]{
    		\begin{minipage}[b]{0.465\linewidth}
  		 	\includegraphics[width=0.85\linewidth]{noisy_rmse.jpg}
    		\end{minipage}
    	}
	\end{center}
% 	\vspace{-.2in}
	\caption{\textbf{Ablation Study}. Average RMSE values for depth image super-resolution. The low-resolution depth image are obtained by (a): Nearest-neighbour downsampling, (b): Bicubic downsampling and Gaussian noise.}
	\label{fig:cd}
\end{figure}

==> Deep Attentional Guided Image Filtering/fig_flash.tex <==
\begin{figure*}[!tb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{cs_guide.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Target]{
    		\begin{minipage}[b]{0.1385\linewidth}
  		 	\includegraphics[width=1\linewidth]{cs_input.jpg}
    		\end{minipage}
    		\hspace{-0.09in}
    	}\subfigure[SDF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{cs_sdf.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[RTV]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{cs_ours.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DJFR]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{cs_djfr.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DKN]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{cs_dkn.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{cs_dagf1.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}
	\end{center}
% 		\vspace{-0.1in}
	\caption{Visual comparison of cross-modality image restoration. Top: flash guided non-flash image denoising. Bottom: NIR guided color image denoising. (a): Guidance image, (b): Target image, (c): SDF~\cite{sdf}, (d): RTV~\cite{RTV}, (e): DJFR~\cite{DJFR}, (f): DKN~\cite{DKN}, (f): DAGF. Please enlarge the PDF for more details.}
	\label{fig:flash}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig_noisy.tex <==
\begin{figure*}[!tb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_RGB.jpg} 
		\end{minipage}
		\hspace{-0.1in}
		\vspace{-0.2in}
	}\subfigure[Target]{
    		\begin{minipage}[b]{0.1958\linewidth}
  		 	\includegraphics[width=1\linewidth]{ns_BIC.jpg}
    		\end{minipage}
    		\hspace{-0.1in}
    	}\subfigure[GF]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_GF.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[MUF]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_MUF.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[SDF]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_sdf.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}
	\subfigure[PAC]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_PacNet.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[DJFR]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_DJFR.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[DKN]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_DKN.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_DAGF1.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[GT]{
		\begin{minipage}[b]{0.1958\linewidth}
			\includegraphics[width=1\linewidth]{ns_GT.jpg} 
		\end{minipage}
	}
	\end{center}
% 		\vspace{-0.1in}
	\caption{Qualitative comparison of joint depth map super-resolution and denoising. Please enlarge the PDF for more details. (a): Guidance Image, (b): Target image, (c): GF~\cite{GF}, (d): MUF~\cite{mugf}, (e): SDF~\cite{sdf}, (f): PAC~\cite{PanNet}, (g): DJFR~\cite{DJFR}, (h): DKN~\cite{DKN}, (i): DAGF and (j): Ground-truth image. ease enlarge the PDF for more details.}
	\label{fig:fig_noisy}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig_real.tex <==
\begin{figure*}[!tb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{rgb_tof.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Target]{
    		\begin{minipage}[b]{0.1385\linewidth}
  		 	\includegraphics[width=1\linewidth]{bic_tof.jpg}
    		\end{minipage}
    		\hspace{-0.09in}
    	}\subfigure[SDF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{sd_tof.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DGDIE]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{dg_tof.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DKN]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{dkn_tof.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{dagf_tof.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[GT]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{gt_tof.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}
	\end{center}
% 	\vspace{-0.1in}
	\caption{Visual comparison of realistic depth map super-resolution on two examples (\textit{books} and \textit{devil}) from ToFMark~\cite{TGV} dataset: (a): Guidance image, (b): Target image, (c): SDF~\cite{sdf}, (d): DGDIE~\cite{gu2017learning}, (e): DKN~\cite{DKN}, (f): DAGF, (e): Ground truth. Please enlarge the PDF for more details.}
	\label{fig:fig_real}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig_sal.tex <==
\begin{figure*}[!htb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_rgb.jpg} 
		\end{minipage}
	}\subfigure[Bicubic]{
    		\begin{minipage}[b]{0.114\linewidth}
  		 	\includegraphics[width=1\linewidth]{sod_bic.jpg}
    		\end{minipage}
    	}\subfigure[DMSG]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_DMSG.jpg} 
		\end{minipage}
% 		\hspace{-0.1in}
	}\subfigure[DJFR]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_DJFR.jpg} 
		\end{minipage}
	}\subfigure[PAC]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_PacJointUpsample.jpg} 
		\end{minipage}
	}\subfigure[DKN]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_DKN.jpg} 
		\end{minipage}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_DAGF.jpg} 
		\end{minipage}
	}\subfigure[GT]{
		\begin{minipage}[b]{0.114\linewidth}
			\includegraphics[width=1\linewidth]{sod_GT.jpg} 
		\end{minipage}
	}
	\end{center}
% 	\vspace{-0.1in}
	\caption{Visual comparison of $8\times$ saliency map super-resolution on the DUT-OMRON dataset~\cite{DUT}: (a): Guidance, (b): low-resolution image, (c): DMSG~\cite{DMSG}, (d): DJFR~\cite{DJFR}, (e): PAC~\cite{PanNet}, (f): DKN~\cite{DKN}, (e): DAGF, (h): Ground truth. Please enlarge the PDF for more details.}
	\label{fig:fig_sal}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig_seg.tex <==
\begin{figure*}[!htb]
	\begin{center}
		\subfigure[RGB Image]{
		\begin{minipage}[b]{0.155\linewidth}
			\includegraphics[width=1\linewidth]{seg_rgb_img.jpg} 
		\end{minipage}
	}\subfigure[Deeplab-V2]{
    		\begin{minipage}[b]{0.155\linewidth}
  		 	\includegraphics[width=1\linewidth]{seg_base_img.jpg}
    		\end{minipage}
    	}\subfigure[DGF]{
		\begin{minipage}[b]{0.155\linewidth}
			\includegraphics[width=1\linewidth]{seg_dgf_img.jpg} 
		\end{minipage}
	}\subfigure[FDKN]{
		\begin{minipage}[b]{0.155\linewidth}
			\includegraphics[width=1\linewidth]{seg_fdkn_img.jpg} 
		\end{minipage}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.155\linewidth}
			\includegraphics[width=1\linewidth]{seg_dagf_img.jpg} 
		\end{minipage}
	}\subfigure[GT]{
		\begin{minipage}[b]{0.155\linewidth}
			\includegraphics[width=1\linewidth]{seg_gt_img.jpg} 
		\end{minipage}
	}
	\end{center}
% 	\vspace{-0.1in}
	\caption{Visual comparison of semantic segmentation on the validation set of Pascal VOC 2012 dataset~\cite{VOC}. (a): RGB image, (b): Deeplab-V2~\cite{DeepLab}, (c): DGF~\cite{DGF}, (d): FDKN~\cite{DKN}, (e): DAGF, (f): ground truth image.  Please enlarge the PDF for more details.}
	\label{fig:seg_fig}
\end{figure*}

==> Deep Attentional Guided Image Filtering/fig_tr.tex <==
\begin{figure*}[!htb]
	\begin{center}
		\subfigure[Target]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{tr_input.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[RTV]{
    		\begin{minipage}[b]{0.1385\linewidth}
  		 	\includegraphics[width=1\linewidth]{tr_rtv.jpg}
    		\end{minipage}
    		\hspace{-0.09in}
    	}\subfigure[RGF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{tr_rgf.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[SDF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{tr_sdf.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DJFR]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{tr_djf.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DKN]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{tr_dkn.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[DAGF]{
		\begin{minipage}[b]{0.1385\linewidth}
			\includegraphics[width=1\linewidth]{tr_dagf1.jpg} 
		\end{minipage}
	}
	\end{center}
% 	\vspace{-0.1in}
	\caption{Visual comparisons of texture remove results. (a): Target image, (b): RTV~\cite{RTV}, (c): RGF~\cite{RGF}, (d): SDF~\cite{sdf}, (e): DJFR~\cite{DJFR}, (f): DKN~\cite{DKN}, (g): DAGF. Please enlarge the PDF for more details.}
	\label{fig:tr}
\end{figure*}

==> Deep Attentional Guided Image Filtering/jsd.tex <==
\begin{table*}[!tb]\setlength{\tabcolsep}{10pt}\renewcommand{\arraystretch}{1.2}
	\begin{center}
	\caption{\label{tab:jsd_result} Quantitative comparison for joint depth image super-resolution and denoising on four standard RGB/D datasets in terms of average RMSE values. Following the experimental setting of \cite{DJF, DKN}), we calculate the average RMSE values in cenrimeter for NYU v2~\cite{NYU} dataset. For other datasets, we compute the RMSE values by scaling the depth value to the range [0, 255]. The best performance for each case are highlighted in \textbf{boldface} while the second best ones are \underline{underscored}. For RMSE metric, the lower values mean the better performance.}
		\begin{tabular}{lccccccccccccccc}
		\toprule
		{Datasets} & \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{Lu} & \multicolumn{3}{c}{NYU v2} &  \multicolumn{3}{c}{Sintel} \\
		\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
		{Method}  &$4\times$ & $8 \times$  & $16\times$  & $4\times$ & $8 \times$  & $16\times$  &$4\times$ & $8 \times$  & $16\times$ &$4 \times$ & $8 \times$  & $16\times$\\
		\midrule
		DGF~\cite{DGF} & 2.70 & 4.13 & 6.38 & 4.06 & 5.85 & 8.39 & 6.52 & 9.23 & 13.00 & 6.94 & 9.03 & 12.05 \\
		DJF~\cite{DJF} & 1.80 &  2.99 &  5.16 & 1.85 &  3.13 &  5.39 & 3.74 &  5.95 &  9.61 & 4.88 &  6.93 &  10.05 \\
		DMSG~\cite{DMSG} & 1.79 &  2.69 &  4.75 & 1.88 &  \underline{2.79} &  4.84 & 3.60 &  5.31 &  \underline{8.07} & 4.74 &  6.36 &  \underline{8.72} \\
		DJFR~\cite{DJFR} &1.86 &  3.07 &  5.27 & 1.91 &  3.21 &  5.51 & 4.01 &  6.21 &  9.90 & 5.10 &  7.12 &  10.23  \\
		DSRN~\cite{DepthSR} & 1.84 &  2.99 &  4.70 & 1.97 &  2.98 &  5.94 & 4.36 &  6.31 &  9.75 & 5.49 &  7.21 &  9.80 \\
		PAC~\cite{PanNet} & 1.81 & 2.94 & 5.08 & 1.93 & 3.44 & 6.18 & 4.23 & 6.24 & 9.54 & 5.40 & 7.32 & 9.89 \\
		DKN~\cite{DKN} &\underline{1.76} &  \underline{2.68} &  \underline{4.55} & \underline{1.81} &  2.82 &  \underline{4.81} & \underline{3.39} &  \underline{5.24} &  8.41 & \underline{4.51} &  \underline{6.25} &  9.20 \\
		DAGF (Ours) & \textbf{1.72} &  \textbf{2.61} &  \textbf{4.24} & \textbf{1.74} &  \textbf{2.72} &  \textbf{4.51} & \textbf{3.25} &  \textbf{5.01} & \textbf{7.54} & \textbf{4.42} &  \textbf{6.09} & \textbf{8.25} \\
		\bottomrule
		\end{tabular}
	\end{center}
\end{table*}

==> Deep Attentional Guided Image Filtering/tab1.tex <==
\begin{table*}[!t]\setlength{\tabcolsep}{10pt}\renewcommand{\arraystretch}{1.2}
	\begin{center}
	\caption{\label{tab:nyu_result} Quantitative comparison for depth image super-resolution on four standard RGB/D datasets in terms of average RMSE values. Following the experimental setting of~\cite{DJF, DKN}, we calculate the average RMSE values in cenrimeter for NYU v2~\cite{NYU} dataset. For other datasets, we compute the RMSE values by scaling the depth value to the range [0, 255]. The best performance for each case are highlighted in \textbf{boldface} while the second best ones are \underline{underscored}. For RMSE metric, the lower values mean the better performance.}
		\begin{tabular}{lcccccccccccc}
		\toprule
		{Datasets} & \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{Lu} & \multicolumn{3}{c}{NYU v2} &  \multicolumn{3}{c}{Sintel} \\
		\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
		{Method}  &$4\times$ & $8 \times$  & $16\times$  & $4\times$ & $8 \times$  & $16\times$  &$4\times$ & $8 \times$  & $16\times$ &$4 \times$ & $8 \times$  & $16\times$\\
		\midrule
		Bicubic & 4.44 & 7.58 & 11.87 & 5.07 & 9.22 & 14.27 & 8.16 & 14.22 & 22.32  & 10.11 & 14.51 & 19.95 \\
		MRF~\cite{MRF} & 4.26 & 7.43 & 11.80 & 4.90 & 9.03 & 14.19 & 7.84 & 13.98 & 22.20 &9.87& 13.45& 18.19  \\
		GF~\cite{GF}) & 4.01 & 7.22 & 11.70 & 4.87 & 8.85 & 14.09 & 7.32 & 13.62 & 22.03  & 8.83 & 12.60 & 18.78 \\		
		TGV~\cite{TGV}) & 3.39 & 5.41 & 12.03 & 4.48 & 7.58 & 17.46 & 6.98 & 11.23 & 28.13 & 8.30 & 13.05 & 19.96  \\
% 		Park~\citep{Park} & 2.82 & 4.08 & 7.26 & 4.09 & 6.19 & 10.14 & 5.21 & 9.56 & 18.10 \\
		SDF~\cite{sdf}) & 3.14 & 5.03 & 8.83 & 4.65 & 7.53 & 11.52 & 5.27 & 12.31 & 19.24 & 9.20& 13.63& 19.36 \\
		FBS~\cite{FBS}) & 2.58&  4.19 & 7.30&  3.03 & 5.77&  8.48 & 4.29 & 8.94 & 14.59 & 8.29& 10.31& 16.18\\
		JBU~\cite{JBU}) & 2.44 & 3.81 & 6.13 & 2.99 & 5.06 & 7.51 & 4.07 & 8.29 & 13.35 &8.25& 11.74& 16.02  \\
		\multicolumn{10}{l}{Experiment results for depth map super-resolution (Nearest-neighbour down-sampling).}  \\
		DGF~\cite{DGF}) & 3.92& 6.04& 10.02& 2.73& 5.98& 11.73& 4.50& 8.98& 16.77& 7.53& 11.53& 17.50  \\
		DJF~\cite{DJF}) & 2.14 & 3.77 & 6.12 & 2.54 & 4.71 & 7.66 & 3.54 & 6.20 & 10.21 & 7.09& 9.12& 12.36 \\
		DMSG~\cite{DMSG}) &  \underline{1.79} & 3.39 & 5.87 & 2.48 & 4.74 & 7.51 & 3.48 & 6.07 & 10.27 & 6.80& 9.09& 11.81 \\
		DJFR~\cite{DJFR}) & 1.98 & 3.61 & 6.07 &  \underline{2.22} &  4.54 & 7.48 & 3.38 & 5.86 & 10.11 &7.05& 9.12& 12.61 \\
		DSRN~\cite{DepthSR}) & 2.08 &  3.26 &  5.78 & 2.57 &  4.46 &  6.45 & 3.49 &  5.70 &  9.76 & 7.29 &  9.43 &  11.62  \\
		PAC~\cite{PanNet}) & 1.91 & 3.20 & 5.60 & 2.48 & 4.37 & 6.60 & 2.82 & 5.01 & 8.64 &6.79& \underline{8.36} & \underline{11.02} \\
		DKN~\cite{DKN}) & 1.93 &  \underline{3.17} &  \underline{5.49} & 2.35 & \underline{4.16} & \underline{6.33} &  \underline{2.46} &  \underline{4.76} &  \underline{8.50}  & \underline{6.84} & 8.61& 11.21 \\
		DAGF(Ours) & \textbf{1.78}& \textbf{2.73}&\textbf{4.75}& \textbf{1.96}& \textbf{3.81}& \textbf{6.16}& \textbf{2.35}& \textbf{4.62}& \textbf{7.81}& \textbf{6.72}& \textbf{8.35}& \textbf{10.64}  \\
		\multicolumn{10}{l}{Experiment results for depth map super-resolution (Bicubic down-sampling).}  \\
		DGF~\cite{DGF})  & 1.94 & 3.36 & 5.81 & 2.45 & 4.42 & 7.26 & 3.21 & 5.92 & 10.45 & 5.91 & 8.02 & 11.17  \\
		DJF~\cite{DJF}) & 1.68 & 3.24 & 5.62 & 1.65 & 3.96 & 6.75 & 2.80 & 5.33 & 9.46 & 5.30 & 7.53 & 10.41 \\
		DMSG~\cite{DMSG}) & 1.88 & 3.45 & 6.28 & 2.30 & 4.17 & 7.22 & 3.02 & 5.38 & 9.17 & 4.73& 6.26 & \underline{8.36} \\
		DJFR~\cite{DJFR}) & 1.32 & 3.19 & 5.57 & 1.15 & 3.57 & 6.77 & 2.38 & 4.94 & 9.18 & 4.90 & 7.39 & 10.33\\
		DSRN~\cite{DepthSR}) & 1.77 &  3.05 &  4.96 & 1.77 &  3.10 &  \underline{5.11} & 3.00 &  5.16 &  8.41 & 4.49 &  6.53 &  9.28 \\
		PAC~\cite{PanNet}) &  1.32 & 2.62 & 4.58 & 1.20 & 2.33 & 5.19 & 1.89 & 3.33 & 6.78 & 4.42 & 6.13 & 8.42\\
		DKN~\cite{DKN}) &  \underline{1.23} & \underline{2.12} &\underline{4.24} & \underline{0.96} & \underline{2.16} & \underline{5.11} & \underline{1.62} & \underline{3.26} & \underline{6.51} & \underline{4.38} & \underline{5.89}  & 8.40  \\
		DAGF(Ours) & \textbf{1.15} & \textbf{1.80}& \textbf{3.70} & \textbf{0.83} & \textbf{1.93} & \textbf{4.80} & \textbf{1.36} & \textbf{2.87} & \textbf{6.06} & \textbf{3.84} &\textbf{5.59} & \textbf{7.44}  \\
% 		\multicolumn{10}{l}{Experiment results for depth map super-resolution (bicubic down-sampling and gaussian noisy).}  \\
% 		DGF~(Wu et al., \cite{DGF}) & 2.70 & 4.13 & 6.38 & 4.06 & 5.85 & 8.39 & 6.52 & 9.23 & 13.00 & 6.94 & 9.03 & 12.05 \\
% 		DJF~(Li et al., \cite{DJF}) & 1.80 &  2.99 &  5.16 & 1.85 &  3.13 &  5.39 & 3.74 &  5.95 &  9.61 & 4.88 &  6.93 &  10.05 \\
% 		DMSG~(Hui et al., \cite{DMSG}) & 1.79 &  2.69 &  4.75 & 1.88 &  \underline{2.79} &  4.84 & 3.60 &  5.31 &  \underline{8.07} & 4.74 &  6.36 &  \underline{8.72} \\
% 		DJFR~(Li et al., \cite{DJFR}) &1.86 &  3.07 &  5.27 & 1.91 &  3.21 &  5.51 & 4.01 &  6.21 &  9.90 & 5.10 &  7.12 &  10.23  \\
% 		DSRN~(Guo et al., \cite{DepthSR}) & 1.84 &  2.99 &  4.70 & 1.97 &  2.98 &  5.94 & 4.36 &  6.31 &  9.75 & 5.49 &  7.21 &  9.80 \\
% 		PAC~(Su et al., \cite{PanNet}) & 1.81 & 2.94 & 5.08 & 1.93 & 3.44 & 6.18 & 4.23 & 6.24 & 9.54 & 5.40 & 7.32 & 9.89 \\
% 		DKN~(Kim et al., \cite{DKN}) &\underline{1.76} &  \underline{2.68} &  \underline{4.55} & \underline{1.81} &  2.82 &  \underline{4.81} & \underline{3.39} &  \underline{5.24} &  8.41 & \underline{4.51} &  \underline{6.25} &  9.20 \\
% 		DAGF (Ours) & \textbf{1.72} &  \textbf{2.61} &  \textbf{4.24} & \textbf{1.74} &  \textbf{2.72} &  \textbf{4.51} & \textbf{3.25} &  \textbf{5.01} & \textbf{7.54} & \textbf{4.42} &  \textbf{6.09} & \textbf{8.25} \\
		\bottomrule
		\end{tabular}
	\end{center}
\end{table*}

==> Deep Attentional Guided Image Filtering/tab_abl.tex <==
\begin{table*}[!htb]\setlength{\tabcolsep}{7.5pt}\renewcommand{\arraystretch}{1.2}
    \begin{center}
        \caption{\label{tab_abl} \textbf{Ablation Study}. Quantitative comparison of different components for $16\times$ depth image super-resolution. We chose RMSE as the evaluation metric, and the lower values indicate better performance. Model7 is our final model (DAGF).}
        \begin{tabular}{lcccccccccccccc}
        \toprule
         \multirow{2}{*}{Model} & \multicolumn{2}{l}{Kernel Generation}  & \multicolumn{3}{l}{Kernel Combination} & \multirow{2}{*}{$\mathcal{L}_{ms}$}& \multirow{2}{*}{$\mathcal{L}_{ba}$} &  \multirow{2}{*}{Middlebury}  & \multirow{2}{*}{Lu}  & \multirow{2}{*}{NYU v2} & \multirow{2}{*}{Sintel} & \multirow{2}{*}{Average} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-6}
        ~ & Target & Guidance & MUL & SUM & AKL & ~& ~ &   \\ 
        \midrule
       Model1 & $\checkmark$ &  & & ~& & & & 7.08& 7.87& 11.99& 13.67 & 10.15 \\
       Model2 &~ & $\checkmark$ & & ~& & &  & 5.68& 7.19& 9.09& 11.82 & 8.45 \\
       Model3  &  $\checkmark$ & $\checkmark$ & $\checkmark$ & & & & & 5.47 & 6.84 & 9.07 & 11.74 & 8.28\\ 
       Model4  &  $\checkmark$ & $\checkmark$ & ~ & $\checkmark$ &  & && 5.36& 6.90&  8.99& 11.65 & 8.23\\ 
       Model5 &  $\checkmark$ & $\checkmark$ & ~ & ~ &  $\checkmark$ & & &  5.06& 6.57& 8.49& 11.18 & 7.82 \\ 
       Model6 &  $\checkmark$ & $\checkmark$ & ~ & ~ &  $\checkmark$ & $\checkmark$ & & 4.88 & 6.19& 7.92& 10.89 & 7.47\\ 
       Model7 &  $\checkmark$ & $\checkmark$ & ~ & ~ &  $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{4.75} & \textbf{6.16}& \textbf{7.81} & \textbf{10.64} & \textbf{7.34} \\ 
    \bottomrule
    \end{tabular}
    \end{center}
\end{table*}

==> Deep Attentional Guided Image Filtering/tab_ba.tex <==
\begin{figure*}[!tb]
	\begin{center}
		\subfigure[Guidance]{
		\begin{minipage}[b]{0.195\linewidth}
			\includegraphics[width=1\linewidth]{ba_rgb.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[Target]{
    		\begin{minipage}[b]{0.195\linewidth}
  		 	\includegraphics[width=1\linewidth]{ba_bic.jpg}
    		\end{minipage}
    		\hspace{-0.09in}
    	}\subfigure[w/o $\mathcal{L}_{ba}$]{
		\begin{minipage}[b]{0.195\linewidth}
			\includegraphics[width=1\linewidth]{ba_m6.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[w/ $\mathcal{L}_{ba}$]{
		\begin{minipage}[b]{0.195\linewidth}
			\includegraphics[width=1\linewidth]{ba_m7.jpg} 
		\end{minipage}
		\hspace{-0.09in}
	}\subfigure[GT]{
		\begin{minipage}[b]{0.195\linewidth}
			\includegraphics[width=1\linewidth]{ba_gt.jpg} 
		\end{minipage}
	}
	\end{center}
	\vspace{-.1in}
	\caption{\textbf{Ablation Study}. Visual comparison of an example without and with the proposed boundary-aware loss for depth image super-resolution. Please enlarge the PDF for more details.}
	\label{fig:abl_baloss}
\end{figure*}

==> Deep Attentional Guided Image Filtering/tab_ecl.tex <==
\begin{figure}[!tb]
	\begin{center}
		\subfigure[Train]{
		\begin{minipage}[b]{0.47\linewidth}
			\includegraphics[width=1\linewidth]{train_rmse.jpg} 
		\end{minipage}
		\hspace{-0.1in}
	}\subfigure[Test]{
    		\begin{minipage}[b]{0.458\linewidth}
  		 	\includegraphics[width=1\linewidth]{test_rmse.jpg}
    		\end{minipage}
    	}
	\end{center}
% 	\vspace{-.2in}
	\caption{\textbf{Ablation Study}. Training and testing RMSE values on NYU v2 dataset~(Silberman et al., \cite{NYU}) for $16\times$ depth image super-resolution. MS denotes the proposed multi-stage loss $\mathcal{L}_{ms}$.}
	\label{fig:ecl}
\end{figure}

==> Deep Attentional Guided Image Filtering/tab_kernel.tex <==
\begin{table}[!tb]\setlength{\tabcolsep}{10pt}\renewcommand{\arraystretch}{1.2}
    \begin{center}
        \caption{\label{tab:tab_kernel}\textbf{Ablation study}. Quantitative comparison of different size of kernel ($k\times k$) and the number of pyramid level ($m$).}
        \begin{tabular}{lcccc}
        \toprule
        Kernel Size & $m = 1$ & $m = 2$ & $m = 3$  & $m = 4$  \\
        \midrule
        $1 \times 1$ & 12.8 & 11.72 & 11.41 & 11.26 \\
        $3 \times 3$ & 8.97 & 8.12 & 7.81 & 7.75 \\
        $5 \times 5$ & 8.60 & 8.02 & 7.73 & 7.98\\
        $7 \times 7$ & 8.67 & 7.94 & 7.78 & 7.99\\
    \bottomrule
    \end{tabular}
    \end{center}
    We report average RMSE values of the last 449 image pairs in NYU v2 dataset~\cite{NYU}.
\end{table}

==> Deep Attentional Guided Image Filtering/tab_real.tex <==
\begin{table}[!htb]\setlength{\tabcolsep}{12pt}\renewcommand{\arraystretch}{1.2}
    \begin{center}
    \caption{\label{tab:tab_real}Quantitative comparison for realistic depth image super-resolution in terms of RMSE values on the ToFMark~\cite{TGV} dataset. The best performance for each case are highlighted in \textbf{boldface} while the second ones are \underline{underscored}.}
         \begin{tabular}{lccc}
        \toprule
        Methods & Books & Devil & Shark \\
            \midrule
        Bilinear & 17.10 & 20.17 & 18.66 \\
        JBU~\cite{JBU} & 16.03 & 18.79 & 27.57 \\
        GF~\cite{GF} & 15.74 & 18.21 & 27.04 \\
        TGV~\cite{TGV} & 12.36 & 15.29 & 14.68 \\
        SDF~\cite{sdf}  & 12.66 & 14.33 & 10.68 \\
        Yang~\cite{2015Color} & 12.25 & 14.71 & 13.83 \\
        DGDIE~\cite{gu2017learning} & 12.32 & 14.06 & 9.66 \\
        DKN~\cite{DKN} & \underline{11.81} & \underline{13.54} & \underline{9.11} \\
        DAGF (Ours) & \textbf{11.80} & \textbf{13.47} & \textbf{9.07} \\
    \bottomrule
    \end{tabular}
    \end{center}
\end{table}

==> Deep Attentional Guided Image Filtering/tab_sal.tex <==
\begin{table*}[!htp]\setlength{\tabcolsep}{12pt}\renewcommand{\arraystretch}{1.2}
    \begin{center}
        \caption{\label{tab:tab_sal}Quantitative comparison of $8 \times$ saliency map super-resolution on the DUT-OMRON dataset~\cite{DUT}. Following DJFR~ \cite{DJFR}, we use F-measure to calculate the difference between the predicted saliency map and the corresponding ground-truth. The best performance for each case is highlighted in \textbf{boldface} while the second one is \underline{underscored} For F-measure, the higher values mean the better performance.}
        \begin{tabular}{ccccccccc}
        \toprule
        Methods & Bicubic & GF~\cite{GF} &  DMSG~\cite{DMSG} & DJFR~\cite{DJFR} & PAC~\cite{PanNet} & FDKN~\cite{DKN} & DKN~\cite{DKN} & DAGF (Ours) \\
        \midrule
        Fscore &  0.853 & 0.821 & 0.910 & 0.901 & 0.922 & 0.921& \underline{0.926} & \textbf{0.932} \\
    \bottomrule
    \end{tabular}
    \end{center}
\end{table*}

==> Deep Attentional Guided Image Filtering/tab_seg.tex <==
\begin{table}[!tb]\setlength{\tabcolsep}{25pt}\renewcommand{\arraystretch}{1.2}
    \begin{center}
         \caption{\label{tab:tab_seg}Quantitative comparison for semantic segmentation in terms of average IoU on the validation set of Pascal VOC 2012. The best performance for each case are highlighted in \textbf{boldface} while the second ones are \underline{underscored}.}
         \begin{tabular}{lc}
        \toprule
        Methods & Mean IoU \\
            \midrule
            Deeplab-V2~\cite{DeepLab}& 70.69  \\
            DenseCRF~\cite{CRF} & 71.98 \\
            DGF~\cite{DGF} & 72.96 \\
            DJFR~\cite{DJFR} & 73.30  \\
            FDKN~\cite{DKN} & \underline{73.60} \\
            DAGF (Ours) & \textbf{73.76} \\
    \bottomrule
    \end{tabular}
    \end{center}
\end{table}

==> Deep Attentional Guided Image Filtering/time_rmse.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{time_rmse.jpg}
    \caption{Average runtime (in seconds) and root mean square error (RMSE) comparison for $16 \times$ depth image super-resolution on NYU v2 dataset~\cite{NYU}. All the runtimes are evaluated on the same NVIDIA 1080Ti GPU with depth image size $480 \times 640$.}
    \label{fig:time_rmse}
\end{figure}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

